New Methods for Detecting Concentric Objects With High Accuracy

Fitting concentric geometric objects to digitized data is an important problem in many areas such as iris detection, autonomous navigation, and industrial robotics operations. There are two common approaches to fitting geometric shapes to data: the geometric (iterative) approach and algebraic (non-iterative) approach. The geometric approach is a nonlinear iterative method that minimizes the sum of the squares of Euclidean distances of the observed points to the ellipses and regarded as the most accurate method, but it needs a good initial guess to improve the convergence rate. The algebraic approach is based on minimizing the algebraic distances with some constraints imposed on parametric space. Each algebraic method depends on the imposed constraint, and it can be solved with the aid of the generalized eigenvalue problem. Only a few methods in literature were developed to solve the problem of concentric ellipses. Here we study the statistical properties of existing methods by firstly establishing a general mathematical and statistical framework for this problem. Using rigorous perturbation analysis, we derive the variances and biasedness of each method under the small-sigma model. We also develop new estimators, which can be used as reliable initial guesses for other iterative methods. Then we compare the performance of each method according to their theoretical accuracy. Not only do our methods described here outperform other existing non-iterative methods, they are also quite robust against large noise. These methods and their practical performances are assessed by a series of numerical experiments on both synthetic and real data.

==> somereadyslides.tex <==
\begin{frame}
\frametitle{\textbf{Desirable Statistical properties}}
\begin{enumerate}
\vspace{-3mm}
 \item<1-> \textbf{Consistency:}
 \begin{itemize}
\item <2->\textbf{Traditional approach}: Used in econometric and sociology, etc.
 $$\lim_{\R n\rightarrow \infty}\hbtheta(\bx_1,\cdots,\bx_n)\stackrel{\rm P}{=}\bbtheta \text{ (the true value of $\btheta$)}$$
\item <2-> \textbf{Small noise approach}: Used in computer vision and image processing applications.
    $$\lim_{\B \sigma\rightarrow 0}\hbtheta(\bx_1,\cdots,\bx_n)\stackrel{\rm P}{=}\bbtheta $$
\end{itemize}
\vspace{-3mm}
 \item<3-> \textbf{Unbiasedness}: \emph{$\hbtheta$ is unbiased} if it does not systematically overestimate or underestimate $\bbtheta$, i.e.,  $\IE(\hbtheta)= \bbtheta$.
 \item<4-> \textbf{Efficiency:} \emph{$\hbtheta$ is efficient} if its variance attains its natural bound.
\item<5-> \textbf{ Our criterion is Mean Square Error (MSE):}
$$\IE[(\hbtheta-\tbtheta)(\hbtheta-\tbtheta)^T]={\rm Var}(\hbtheta)+{\rm Bias}(\hbtheta){\rm Bias}(\hbtheta)^T, \text{ where } {\rm Bias}(\hbtheta)=\IE(\hbtheta)-\tbtheta $$

 \end{enumerate}
 \end{frame}
 \section{Error Analysis}
\begin{frame}

\begin{center}
{\B {\Huge \textbf{Error Analysis}} \\
{\Large \textbf{general scheme}\\
\cite{AC4,ACKS1,ACKS2}}
 }
 \end{center}
\end{frame}
%--------------------------------
\begin{frame}
\begin{beamerboxesrounded}[upper=uppercol,lower=lowercol,shadow=true]{}
\begin{theorem}[Al-Sharadqah and Chernov \cite{AC1}]
Suppose one is fitting curves defined by {\R \emph{an implicit equation}}
$$\bG(x,y,\btheta)=0,\quad \hat{\btheta}_{\rm Q}=\tilde{\btheta} +\Delta_1 \hat{\btheta}+ \Delta_2
\hat{\btheta}$$
then
\begin{align*}{\rm MSE}(\hat{\btheta})&=\underset{\cO( \sigma^2/n)}{\underbrace{{\rm Var}(\hat{\btheta}_{Q})}}
+\underset{\cO(\sigma^4)}{\underbrace{{\rm Bias}(\hat{\btheta}_{\rm Q}){\rm Bias}(\hat{\btheta}_{\rm Q})^T}}+\cdots\\
&=\cO(\sigma^2/n) + \cO(\sigma^4) +\cO(\sigma^4/n)+\cO(\sigma^4/n^2)  + \cO(\sigma^6)
\end{align*}
where $$
{\rm Bias}(\hbtheta_{\rm Q})=\underset{\text{Essential bias}}{\underbrace{ \sigma^2\bB_1}}+\underset{\text{Nonessential bias}}{\underbrace{ \sigma^2\bB_2}}\sim \sigma^2+\frac{\sigma^2}{n}$$
 \end{theorem}
 \end{beamerboxesrounded}
\end{frame}
 %----
\begin{frame}
\frametitle{\textbf{Classification of high order terms}}

 \begin{block}<+->{The order of magnitude, Amemiya \& Wayne Fuller 1988)}
\begin{table}
\begin{center}
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{|c|cccc|}
\hline  & $\phantom{m}\sigma^2/n\phantom{m}$ &
        $\phantom{m}\sigma^4\phantom{m}$ & $\phantom{m}\sigma^4/n\phantom{m}$ &
        $\phantom{m}\sigma^6\phantom{m}$ \\
\hline  small samples ($n\sim 1/\sigma$) & $\sigma^3$ & $\sigma^4$ & $\sigma^5$ & $\sigma^6$ \\
        large samples ($n\sim 1/\sigma^2$) & $\sigma^4$ & $\sigma^4$ &
        $\sigma^6$ & $\sigma^6$ \\ \hline
\end{tabular}
\end{center}
\end{table}
\end{block}
\begin{beamerboxesrounded}[upper=uppercol,lower=lowercol,shadow=true]{}
\begin{theorem}[KCR (Chernov and Lesort 2004)]
For every {\B geometrically consistent estimator $\hbtheta$} of $\btheta$
 $$
   {\rm var}(\hbtheta) \geq\sigma^2 \bD_{\min}, \text{ up to the leading term }
$$
${\rm LHS}\geq {\rm RHS}$ means ${\rm LHS}- {\rm RHS}$ is a positive semi-definite matrix.
\end{theorem}
\end{beamerboxesrounded}
\end{frame}
%-------
\begin{frame}
 \frametitle{\textbf{Error Analysis for circle fitting Problem}}
All algebraic fits solve $\bM\btheta=\lambda\bN\btheta$.
Perturbating each of $\bM$,$\hbtheta$, $\lambda$, and $\bN$ and writing each one as follows:
$$
\bM=\tbM+\Del_1\bM+\Del_2\bM+\cO_{\rm P}(\sigma^3)
$$
\begin{beamerboxesrounded}[upper=uppercol,lower=lowercol,shadow=true]{}
\begin{theorem}[Al-Sharadqah and Chernov \cite{AC1}]
\vspace{-8mm}
\begin{align*}
{\rm Var} (\hat{\btheta}_{\rm Q})&=\frac 1 n\sigma^2\tbM^-\tbM_0\tbM^- \sim \cO(\sigma^2/n),
\quad (\text{here } \tbM_0 \text{ is free of } \bN)\\
{\rm Bias}(\hat{\btheta}_{\rm Q})&=\tbM^-\Bigl(\frac{\tbtheta^T\IE(\bR)\tbtheta}{\tbtheta^T\tbN\tbtheta}\tbN-\IE(\bR)
\Bigr)\tbtheta, \quad \bR=\Del_2\bM-\Del_1\bM\tbM^-\Del_1\bM
\end{align*}
 \vspace{-4mm}
\end{theorem}
\end{beamerboxesrounded}
\end{frame}
\begin{frame}
\frametitle{}
\emph{\small K. Kanatani, P. Rangarajan, Y. Sugaya and H. Niitsuma, HyperLS for parameter estimation in geometric fitting
\emph{Comp. Stat. and Data Analysis}, 55(6), 2011.}
\vspace{7mm}
\begin{beamerboxesrounded}[upper=uppercol,lower=lowercol,shadow=true]{}
\begin{theorem}
\begin{align*}
{\rm Var} (\hat{\btheta}_{\rm Q})&=\frac 1 n\sigma^2\tbM^-\tbM_0\tbM^- \sim \cO(\sigma^2/n),
\quad (\text{here } \tbM_0 \text{ is free of } \bN)\\
{\rm Bias}(\hat{\btheta}_{\rm Q})&=\tbM^-\Bigl(\frac{\tbtheta^T\IE(\bR)\tbtheta}{\tbtheta^T\tbN\tbtheta}\tbN-\IE(\bR)
\Bigr)\tbtheta, \quad \bR=\Del_2\bM-\Del_1\bM\tbM^-\Del_1\bM
\end{align*}
\end{theorem}
\end{beamerboxesrounded}
\begin{block}<2->{\textbf{Remarks:}}
\begin{itemize}
\item<3-> In conic fitting, all algebraic fits do not attain the KCR, i.e., ${\rm Var}(\hbtheta)> \sigma^2\bD_{\rm min}$.
\item<4-> To achieve the KCR, some weights should be considered for each data points
\ \end{itemize}
\end{block}
\end{frame}
